Sharp Analysis for Nonconvex SGD Escaping from Saddle Points

In this paper, we give a sharp analysis for Stochastic Gradient Descent (SGD) and prove that SGD is able to efficiently escape from saddle points and find an $(\epsilon, O(\epsilon^{0.5}))$-approximate second-order stationary point in $\tilde{O}(\epsilon^{-3.5})$ stochastic gradient computations for generic nonconvex optimization problems, when the objective function satisfies gradient-Lipschitz, Hessian-Lipschitz, and dispersive noise assumptions. This result subverts the classical belief that SGD requires at least $O(\epsilon^{-4})$ stochastic gradient computations for obtaining an $(\epsilon,O(\epsilon^{0.5}))$-approximate second-order stationary point. Such SGD rate matches, up to a polylogarithmic factor of problem-dependent parameters, the rate of most accelerated nonconvex stochastic optimization algorithms that adopt additional techniques, such as Nesterov's momentum acceleration, negative curvature search, as well as quadratic and cubic regularization tricks. Our novel analysis gives new insights into nonconvex SGD and can be potentially generalized to a broad class of stochastic optimization algorithms.

==> parts/related_FC.tex <==





%\input{parts/table}







%
%\red{
%Because without Assumption \ref{a5}, SGD can be acted as Gradient Descent,  which,   proven in \cite{du2017gradient},  will take exponential complexity to escape saddles for specific functions.
%  Assumption \ref{a5} is easy to be satisfied by  kinds of  noises, e.g.
%if the noise of the stochastic gradient obeys normal distribution, we have $\tau^2  =  \sigma^2/d$.
% We can also inject  a small independent isotropic noise when accessing the stochastic gradient $\nabla F(\x, \zeta)$ to make  Assumption \ref{a5} hold freely.
%    For example, we can inject a normal noise with distribution satisfying  $N(\mathbf{0}, (\sigma^2/d) \mathbf{I_d})$.
%Then all Assumptions hold  simultaneously with  $\tau^2 = \frac{\sigma^2}{d}$, and the variance $\sigma^2$ being $2$ times larger.
%The obtained algorithm is known as Injected Noisy Stochastic Gradient Descent described in \cite{ge2015escaping}.
% We  also mention the reader that $\frac{\sigma^2}{\tau^2}$ might have dependence on the dimension $d$, e.g.
%for the standard normal noise.
%Thus we cannot treat $\tau$ as a global constant.
%Fortunately, our obtained convergence rate only has logarithmic factors on $\frac{\sigma^2}{\tau^2}$.
% Thus to best of the knowledge, our work is the first dimensional free convergence rate for the standard SGD algorithm\footnote{ In constast, \cite{daneshmand2018escaping} achieves a convergence rate of $\tilde{O}(\tau^{-2}\ep^{-10})$, which has liner dependence on $\tau^{-2}$.} when ignoring poly-logarithmic factors.
%}







